Modelling the Far-Infrared emission in spyral galaxies

This thesis presents an original model for the FIR emission in spirals, developed from an existing radiative transfer code (Bianchi, Ferrara & Giovanardi, 1996, ApJ, 465, 127). The model's main features are: a complete treatment of multiple scattering within geometries appropriate for spirals; a full coverage of spectral range of stellar emission; the use of empirically determined dust properties (some of which are derived in the present work); the production of maps of the dust temperature distribution, together with simulated optical, FIR and sub-millimetre images. The model has been applied to observations of stellar and dust emission in the galaxy NGC 6946. It is found that optically thick models (central face-on optrical depth tau_V \~ 5) are necessary to explain the observed FIR output. For such models, almost 30-40% of the intrinsic starlight is absorbed. The observed ratio of FIR and optical scalelengths can be explained if the dust distribution is more extended than the stellar. However, because of the less steep gradients of optical emission in optically thick cases, a very extended dust distribution is needed (alpha_d ~ 3 alpha_s). The distribution of atomic gas in NGC 6946 has a similar extent. I discuss the approximations in the modelling (mainly the use of smooth distributions against the observed clumpiness of the interstellar medium) and the implications of the results.

==> intro/models.tex <==
\section{Radiative transfer models}

Introduction, it's too difficult to list all the literature models
for the radiative transfer, they are model dependent, we list here only
those that have been applyed to spiral galaxies.

\citet{DisneyMNRAS1989} lists all the easy models, a small introduction
to them, plus a description of the TRIPLEX.

Because of the large albedo (see BFG to be sure about what to write)
scattering is necessary.

Unfortunately it is difficult to produce analytical models with
scattering, if we want to conserve the galactic geometry and we 
have to choose a compromise.

\citet{BruzualApJ1988} have a simple plane parallel geometry, but the
scattering is dealt with in a complete form.

\citet{DiBartolomeoMNRAS1995} for a new procedure, within the same
geometry.

\citet{CorradiMNRAS1996} use a local plane parallel geometry, but with an
exponential distribution. 

\citet{KylafisApJ1987} have a more realistic geometry but scattering was
treated with an approximation.

\citet{ByunApJ1994} uses the same method, generalized to several angles
and including a bulge.

Then I have to stress that it is the best one to find fitting, and all
the papers \citet{XilourisA&A1997,XilourisA&A1998,XilourisSub1998}.

\citet{TrewhellaAAS1998} uses a cellular mode, with its problems, if
there are.

And then the Monte Carlo methods come!

Advantages of the Monte carlo model for the scattering and other things,
see BFG. Disadvantage in the lack of a formula to be used in fitting
like in \citet{XilourisA&A1997,XilourisA&A1998,XilourisSub1998}.

It has been used to simulate stars inside dust clouds.

The first application to galaxies is that of \citet{WittApJ1992},
for spherical geometries.

Then The best model, mine, but not a complete description, that is
deferred to the Sect.~\ref{montecarlo}.

Other Monte Carlo models have been developed by \citet{DeJongA&A1996b}
and \citet{WoodAPJL1997}.

Then an introduction to clumping, the last frontier. It is difficult to
deal with it analitically, exept for simple geometries
\citet{VarosiPrep1999} where the clumping characteristics are described
in a statistical way, therefore the monte carlo is the best way.

A bit of the philosophy of the cellular models, able to fit to several
situation, the works for galaxies in spherical geometries of
\citet{WittSub1999} and for spirals of \citet{KuchinskiAJ1998} and 
\citet{BianchiSub1999}. Modify to find place for \citet{WolfA&A1998b}.

Say that \citet{TrewhellaAAS1998} can deal with clumping, but....

\section{Models of FIR emission}

The energy balance method, explanation, it doesn't give information
about the spectral energy distribution of the dust emission but only on
the total dust emission.

\citet{EvansThesis1992} model 

The different approach of \citet{XuA&A1995}, using scattering and 
a sample of several galaxies.

The \cite{TrewhellaMNRAS1998} implementation on single cells of the
galaxy with the production of extinction maps.

another approach is that of measuring the spectrum of FIR emission, with
the dust temperature, after using a model of dust \citep{MathisA&A1983}, 
or deriving the model
of dust itself \citep{RowanRobinsonMNRAS1992,DesertA&A1990}. 

The model of \citet{DaviesMNRAS1997} produces maps of emission starting
from the distribution of tempearture observed.

Only few models produce their own ISRF from the stellar model and
apply it to a dust distribution

Description of \citet{SilvaApJprep1998} model, too many parameters and
dust coming from the evolutionary model, radiative transfer is an
approximation

Then I should describe what \citet*{SautyA&A1998} do, if I'll ever
understand it. The model is too dependent on the object.


------------------------OLD--------------------

Here a distintion should be made for models of energy balance that
compare only the energy and models that also gives the temperature.

\subsection{\citet{EvansThesis1992} model}

\subsection{\citet{XuA&A1995} model}

\citet{XuA&A1995} compared UV, optical and FIR emission for a 
sample of 135 nearby spiral galaxies with available UV and B fluxes
and 60 and 100$\mu$m IRAS data.

The non-ionizing emission of the stellar component (f$_\mathrm{star}$) 
was derived for 
each galaxy from an extrapolation of the UV and the B-band monocromatic 
fluxes, using synthetic spectra for specific Hubble types and/or UV-optical 
colors. When only IRAS data are available, it is difficult to derive 
the total FIR emission. To overcome this, IRAS data were integrated
with sub-mm observations available for 13 galaxies. In this subsample,
the ratio between the total FIR flux (their f$_\mathrm{dust}$) and the 
FIR flux in the spectral range 40$\mu$m-120$\mu$m, as derived from the  
60 and 100$\mu$m observation (f$_\mathrm{fir}$),
was found to anti-correlate with the ratio between the two IRAS fluxes.
This is expected, since warmer dust (higher 60/100 flux ratio) would emit 
at wavelengths shorter than the 100$\mu$m and most of the radiation 
would be detected by IRAS. For colder dust (lower 60/100 flux ratio), 
the emission would occur out of the IRAS spectral range, and the ratio
f$_\mathrm{dust}$/f$_\mathrm{fir}$ would be larger.

Using this anti-correlation and the available 60 and 100$\mu$m fluxes,
the total dust emission was derived for each galaxy. For their sample,
f$_\mathrm{dust}$/(f$_\mathrm{star}$+f$_\mathrm{dust}$)=0.31, suggesting
that less then one third of the stellar radiation is absorbed by dust.
Ionizing photons are assumed to be absorbed locally, in the HII
regions. The energy absorbed from ionizing photons is derived from 
the H$_\alpha$ fluxes of a subsample of 34 galaxies
and subtracted from the total energy absorbed by dust. Ionizing
photons are extimated to contribute a 14\% and 20\% of the total
dust emission, for early and late type, respectively.

The remaining absorbed energy is then compared to the stellar emission,
using a radiative transfer model in a sandwich geometry, inclusive of
scattering. A mean optical depth $\tau_B=0.60\pm0.05$ is found for the
sample, with larger values for early type galaxies, but still in the
optically thin case. The non-ionizing UV (921\AA$<\lambda<$3650\AA)
is found to dominate the dust heating, contributing to a 60$\pm$9\% of 
the total FIR emission against the 21$\pm$8\% of the optical radiation
(3650\AA$<\lambda<$9000\AA). The rest is due to ionizing photons.

Using the same model, \citet{BuatA&A1996} conduct a more extensive 
analysis on a sligthly larger sample of galaxies (152). The model is
tested for changes in the extinction law, in the UV scattering properties, 
in the synthetic spectra used to estrapolate the UV total emission from 
the monocromatic flux, as well as in the vertical distribution of dust
and stars.
The results are compatible with galaxies being optically thin in the B
band. Since UV, optival and FIR are used to monitor the dust heating and
cooling mechanism, the derived $\tau_B$ is rapresentative of regions
bright in these spectral ranges, like star-forming regions. Being
extinction higher in those regions, $\tau_B$ is likely to be an 
overestimate. They claim that possible selection effects, due to the
sample being UV selected, are not important.
If the dust distribution in a spiral galaxy is peaked in the centre,
the use of a uniform sandwich model would result in an optical depth
that is representative of the mean opacity over all the disk. Their
result could therefore mean that galaxies as a whole are optically thin.
Nevertheless they say that this is not the case: their
affirmation is based on the flat distribution of optically thin dust 
derived by \citep{XuApJ1996b} on M31, using the model of
\citet{XuA&A1995} for several cell on regions of the galactic disk
where resolved sources do not dominated the FIR radiation.

Since UV radiation is the main contributor to the dust heating, it is
possible to derive the recent star-formation rate (on a scale of 10$^8$
years) from FIR observations (note that this is in some way different from
\citet{DevereuxApJL1990} claims, since their UV radiation is processed
as if it was an ISRF).

\citet{XuApJ1996a} measure the ratio between the IRAS 60$\mu$m and
H$_\alpha$ fluxes from bright FIR-resolved sources in M31. Using the
total H$_\alpha$ luminosity and the \citet{DesertA&A1990} dust model, they
extrapolate the fraction of the total FIR luminosity that is associated
with HII regions and star-formation. A value of 30$\pm$14\% is found.

\subsection{\citet{SilvaApJprep1998} model}
There are three dust environment that should be considered in
modelling the extinction effects in the SED of galaxies: 
i) dust in HI clouds heated by the standard ISRF (\textit{cirrus}
component); ii) dust in molecular clouds, associated with star 
formation; iii) circumstellar dust shells.

The intrinsic SED is derived from a model that follows the chemical 
evolution model of galaxies. SED is constructed with a spectral synthesis
technique: given a certain age and metallicity for the galaxy, spectra
of simple population stars are coadded, weighted by the SFR at the time 
of star birth. Circumstellar dust shells around AGB stars are included,
using a model of AGB star evolution that provides the optical and 
geometrical parameters of the shell (as well as mass and other stuff).

They use a three components geometry: i) Molecular clouds with HII and
very young stars (YSO) embedded in it; ii) Stars that have escaped from
molecular clouds; iii) diffuse gas (the \textit{cirrus}: actually the
use this as a dust component only, since there is no mention of gas
emission in the paper).

For the three components they use a double exponential distribution with
the same radial and vertical scalelengths (althought they claim they can
have them different for each component). The vertical scalelength is
0.35 kpc as in the Galaxy (so dust and stars are homogeneously mixed).
The radial scalelength is derived from $M_B$ using an empirical relation
(I believe it's empirical, chech the reference).

For spheroidal galaxies they use a distribution with a King profile for
stars, again assuming a relation between absolute magnitude and the core
radius (a geometrical parameter that defines the distribution, together
with an exponent $\gamma$, that is fixed to 1.5). Dust in
spheroidal system has been suggested to follow a law 
$\rho_{dust}=\rho_{stars}^n$ with n$\approx$ 1/2 - 1/3; this  can be
done with a King model with $gamma$ between 0.5 and 0.75, suggesting 
dust to be less concentrated.

As for the dust model they use the same kind of dust for cirrus and MCs,
allowing for a decrease in PaHs in the latter. Properties of dust in
circumstellar outflows are already included in the spegral synthesis.
The general model is that of Draine and Lee, witha few modification in
graphite particle size distribution to account for MIR emitting grains
(small). PaHs are included.

Knowing the residual gas mass in the galaxy evolution model, the dust
quantity is computed assuming a dust to gas ratio of 1/110 for the
solar metallicity (at other metallicities, tha ratio behaves linearly
with Z)

A fraction f$_{mc}$ of the model gas mas is ascribed to MCs, then the
corresponding dust is subdivided in spherical clouds of 10$^6 M_\odot$
(the molecular clouds radius is a parameter of the model).
Stars are assumed to form in molecular clouds and then they muve
outside. This is mimicked changing the fraction of star energy that is
radiated inside the cloud with time (again the time parameter here is a
model parameter). Radiative transfer in MCs is computed assuming that
all the stars are in the center of the clouds and this leads to high
temperatures (because there is only one \textit{hot spot}).
As a consequence, they use this T as a parameter from which they derive
a lower true maximum T (?????? very vague in the paper).

For what concern radiative transfer in the diffuse ISM, they use an
approximation for scattering, with an effective optical depth that is
the mean of the extinction and absorpion efficiencies (see Rybicky
Lightman). This is rigorous only for an infinite homogeneous medium
and isotropic scattering, but they have checked it gives good results
against Witt at al 1992 models.

The space is divided in a grid and for each volume cell they compute the
contribution from all the other cells, extinguishing by the tau between
the two cells. Finally, looking from a certain direction the total flux
is added, again after extinction due to the distance between the cell 
and the end of the dust distribution has been applied.

Here there is a model for NGC 6946.


==> program/galaxy.tex <==
From their bidimensional model, \citet{DeVaucouleursAJ1978} 
measure a disk radial scalelength $\alpha_\star=3.5$ kpc. The value is
obtained comparing the local ($R_\odot$) vertically integrated surface 
brightness in the B-band (derived from star counts) with the mean central 
surface brightness 21.65 mag arcsec$^{-1}$ for disks of spiral
galaxies~\citep[Freeman Law; ][]{FreemanApJ1970}.

\citet{BahcallApJS1980} built a tridimensional Galactic model to fit
B and V star counts at a Galactic latitude $b>20^\circ$ (where extinction 
is low). The disk component is modelled with an exponential both in the 
radial and in the vertical direction. For $\alpha_\star$ they assume
the \citet{DeVaucouleursAJ1978} value; values for $\beta_\star$ are 
derived from the literature and summarised in a magnitude
(age)-dependent relation: young stars ($M_V<2$) have $\beta_\star=90$ pc,
old disk dwarfs ($M_V>5$) have $\beta_\star=325$ pc, while a linear relation
for stars in the range $2<M_V<5$ is assumed. In this formalism giants 
have $\beta_\star=250$ pc. This model is commonly referred to in the 
literature as the {\em standard model}.
In a subsequent work \citep{BahcallApJS1984} the parameter space is
explored and limits are put on the scalelengths:
$\beta_\star=250\pm100$ pc for giants and $\beta_\star=350\pm50$ pc for 
old disk dwarfs. Although data are poorly sensible to $\alpha_\star$
(because the model is compared to star counts at high latitude), data 
can be reasonably fit only for $\alpha_\star>2.5$ kpc.

A modified \citeauthor{BahcallApJS1980} model is used by
\citet{VanDerKruitA&A1986} to fit the integrated blue and red starlight 
observed by the Background Experiment on board of {\em Pioneer 10}.
To avoid region with high extinction, data for galactic longitude $b>20^\circ$ 
only are used: thus, as shown by the author, only the value 
$\alpha_\star/\beta_\star$ can be derived. Assuming $\beta_\star=325$ pc
a value of $\alpha_\star=5.5$ kpc is derived. As suggested by 
\citet{KentApJ1991} this method is sensitive to local surface brightness 
gradients and may only give a measure of the local exponential scalelength.

\citet*{KentApJ1991} derive the parameters of Galactic structure
from the 2.4-$\mu m$ integrated light as measured from the Infrared
Telescope flown aboard the Space Shuttle during 1985 as a part of the
{\em Spacelab 2} mission. 
A radial exponential distribution is assumed for the disk, allowing for
different vertical distributions.
A correction for extinction (small at this wavelength, although not
negligible) is incorporated in the model, evaluated from the atomic 
hydrogen distribution, assuming a constant value for the dust/hydrogen ratio.
Surface brightness profiles as a function of the galactic longitude at 
several latitudes are compared to the data: the {\em standard model} is 
unable to describe the profile on the galactic plane. 
Using an exponential vertical distribution they find $\beta_\star=204\pm
57$ pc and $\alpha_\star=2.7\pm0.5$ kpc. 
The $\beta_\star$ value is small compared to the \citet{BahcallApJS1980} 
value for the giant star distribution (the main contributor to the 
luminosity in the observed wavelength range). 
For this reason they try a different fit allowing for a varying $\beta_\star$. 
Up to 5.3 kpc they keep $\beta_\star=165$ pc then
they assume a gradient of 30 pc / kpc so that at $R_\odot$
$\beta_\star=247\pm 69$. The corresponding radial scalelengths is
$\alpha_\star=3\pm0.5$ kpc.

We note here that all the works cited up to here used R$_\odot$=8 kpc,
while in the next references the value 8.5 is preferred. When a
scalelength is derived from a model it should be scaled to the value
of  R$_\odot$~\citep{KentApJ1991}.

\citet{WainscoatApJS1992} fit star counts at 12-$\mu m$ and 25-$\mu m$ 
from the {\em IRAS} Point Source Catalog with a Galactic model with
a disk of radial scalelength $\alpha_\star=3.5$ kpc, truncated 
at 15 kpc.
Scaleheights for the vertical exponential distribution are given 
for a a compilation of 87 types of galactic sources responsible for
emission in the NIR bands. Values are similar to those in the 
\citet{BahcallApJS1980} model (e.g. $\beta_\star=325$ pc for 
old dwarfs, 270 pc for giants etc.).
A previous model to fit K-band star count and 12-$\mu m$  IRAS source
count (\citealt{GarwoodPASP1987}, see also \citealt{JonesMNRAS1981})
was using slightly smaller values ($\beta_\star=300$ pc for old disk
dwarfs).

In \citet{RobinA&A1992} the scalelength is measured from B and V-band 
stars counts up to $m_V=25$ mag in a low absorption window in the 
direction of the Galactic anticenter. They use a complex structure and
evolution Galaxy model (the {\em Besan\c{c}on} model): the disk in
this model follows an Einasto density law, that behaves similarly
to an exponential on the radial direction and to a $sech^2$ in the 
vertical. A correction for extinction is evaluated from the U-B/B-V plot 
of a sample of star for which U-band data are available. 
They obtain $\alpha_\star=2.5$ kpc. 
A truncation in the disk at 14-15 kpc is needed to explain
star counts at faint magnitude \citep[see also][]{RobinApJL1992}.

A similar value ($\alpha_\star=2.3\pm0.1$ kpc) is obtained by 
\citet{RuphyA&A1996} using J- and K-band star counts of two
fields in the direction of the Galactic anticenter 
from the Deep Near-Infrared Survey of the Southern Sky. 
The same model as in \citet{RobinA&A1992} is assumed.
Data are corrected for extinction (J-band is sensibly affected)
matching the positions of the observed  and the model J-K colour 
distribution of the stars. The scalelength is obtained minimising the 
difference in shape between the two distributions.
Like in \citet{RobinA&A1992} their fit is not very sensitive on the 
assumed value for $\beta_\star$ (because data are very close to the 
Galactic plane). Again, a truncation at $R_{max}=15\pm2$ kpc is
found.

\citet{PorcelA&A1998} measures $\alpha_\star$ from K-band star counts 
in the Two Micron Galactic Survey database. Extinction effects, low in 
the K-band, are furtherly minimised selecting stars out of the galactic 
plane (at a galactic latitude $b=5^\circ$). A range of galactic longitudes 
($30^\circ<l<70^\circ$) is chosen to minimise the contribution 
to the star distribution of local structures: namely, bulge, ring and bar 
in the centre ($l<30^\circ$) and Local Arm, warp and truncation ($l>70^\circ$).
Contribution from other spiral arms are minimised by the choice of $b$.
In the database, only stars with K-band apparent magnitude $9<m_K<10$
are selected: it can be shown that 80\% of the total light emitted
in this magnitude range is provided by K2-K5III stars, which have 
an absolute magnitude $M_K=-2.5\pm0.6$. Their luminosity function can
thus be conveniently approximated by a Dirac's delta.
They find $\alpha_\star=2.1\pm0.3$ kpc, assuming a vertical scalelength 
$\beta_\star$ of 200 pc (again the result
is nor very sensitive on $\beta_\star$).

These recent results base on star counts are confirmed also by 
the kinematical estimate of \citet{FuxA&A1994}, based on the 
asymmetric drift equation, that gives $\alpha_\star=2.5^{+0.8}_{-0.6}$ kpc,
assuming a constant value for $\beta_\star$. If the gradient in 
$\beta_\star$ derived by \citet{KentApJ1991} is included,
$\alpha_\star=3.1$ kpc. 

Recently \citet*{HaywoodA&A1997a,HaywoodA&A1997b} have questioned the
validity of the exponential assumption for the vertical structure, on
the basis of the {\em Besan\c{c}on} model.  
Rather than adopting different values of $\beta_\star$ for different 
galactic sources, the model derives the vertical structure from the 
combined effect of the star formation history and of the secular heating 
of the disk. After tests on B, V, and I star counts (the \citet{RuphyA&A1996}
value of $\alpha_\star$, 2.5 kpc, is used) they claim that the
exponential is unsuitable to properly describe data for $z<500$ pc. 
They find that the vertical density distribution decreases faster than the
$300-350$ pc generally assumed for old disk dwarf. In \citet{RuphyA&A1996} 
a value of $250$ pc is suggested, as a result of this work. 



==> program/galaxy_old.tex <==
\section{Galactic radial scalelength $\alpha_\star$}
There is a wide range of radial scalelengths in our galaxy:

\citet{PorcelA&A1998} measures $\alpha_\star$ using positions
and K-band magnitudes of stars in the Two Micron Galactic Survey 
database. Extinction effects, low in the K-band, are furtherly
minimized selecting stars out of the galactic plane (at a 
galactic latitude $b=5^\circ$).
Only stars with galactic longitude $l$ between 30$^\circ$ and
70$^\circ$ are used, to minimize the contribution of local structures 
to the star distribution: namely, bulge, ring and bar in the center
($l<30^\circ$) and Local Arm, warp and truncation ($l>70^\circ$).
Contribution from other spiral arms are minimized by the choice of
$b$.
In the database, only stars with K-band apparent magnitude $9<m_K<10$
are selected: it can be shown that 80\% of the total light emitted
in this magnitude range is provided by K2-K5III stars, which have 
an absolute magnitude $M_K=-2.5\pm0.6$. Their luminosity function can
thus be conveniently approximated by a Dirac's delta.
They find $\alpha_\star=2.1\pm0.3$ kpc, assuming a vertical scalelength 
$\beta_\star$ of 200 pc (\citealt{WainscoatApJS1992}; but this result does
not depend on the choice of $\beta_\star$)  and a standard galactocentric
radius for the sun $R_\odot=8.5$ kpc.

\citet{RuphyA&A1996} obtain a similar value ($\alpha_\star=2.3\pm0.1$ kpc),
using J- and K-band data from the Deep Near-Infrared Survey of the 
Southern Sky in the direction of the Galactic anticenter. 
They assume a theoretical luminosity function for the stars and 
a density law for the disk (an Einasto law, that behaves similarly
to an exponential on the radial direction and to a $sech^2$ in the 
vertical; vertical scalelengths in this model depends on the radius).
Data are corrected for extinction (J-band is sensibly affected)
matching the positions of the observed  and the model J-K color 
distribution of the stars. The scalelength is obtained minimizing the 
difference in shape between the two distributions.
Their fit is not very sensitive both on the assumed value for
$\beta_\star$ and on the Star Formation history of their luminosity
function.
Another parameter they derived is the truncation, at $R_{max}=15\pm2$ kpc
($\approx 6.5 \alpha_\star$).

The kinematical extimate of \citet{FuxA&A1994}, based on the 
asymmetric drift equation gives $\alpha_\star=2.5^{+0.8}_{-0.6}$ kpc,
assuming a constant value for $\beta_\star$. If the gradient in 
$\beta_\star$ derived by \citet{KentApJ1991} is included,
$\alpha_\star=3.1 $ kpc. A previous kinematical method gave 4.2, but there
were a few assumptions uncompatible with a vertical exponential
distribution.

\citet*{KentApJ1991} derive the parameters of Galactic structure
from the 2.4-$\mu m$ integrated light as measured from the Infrared
Telescope flown aboard the Space Shuttle during 1985 as a part of the
{\em Spacelab 2} mission. 
Data in this wavelength are better than optical observations because 
of the low (althought not negligible) extinction. Dust emission is
negligible and the contribution from zodiacal light minimal.
They build a model of the Galaxy using a radially exponential disk
and allowing for several vertical behaviour. As starting parameters in
the fit they use $\alpha_\star=3.5$ kpc \citep{DeVaucouleursAJ1978}. 
The theoretical $sech^2$ function for the vertical distribution is 
adopted with a scalelength and $\beta_\star=230-250 pc$ (derived from 
K-band luminosity analysis \citep{GarwoodPASP1987}). In 
\citet{BahcallApJS1980} model, $\beta_\star=250$ pc is the value for 
the giant star distribution (the main contributor to K-band luminosity).
A bulge, modeled as a modified spheroid, is added to model the central
spheroid at $1^\circ < l < 10^\circ$ (no attempt is made to model the 
central cusp and the external part of the speroid for which a two
component spheroid is needed). The minor axis scalelenght of the bulge
is 378 pc with an ellipticity $\epsilon$=0.35. A prominent "hump" of 
emission in the Galactic plane for $10^\circ <l<35^\circ $ is excluded 
from the fit of the exponential disk and is modeled separately with a ring-like
structure.  Extinction is evaluated from the atomic hydrogen distribution, 
assuming a constant value for the dust/hydrogen ratio.

From the Sun position (at $R_\odot=8$ kpc) the model is integrated to
find the surface brightness profile as a funcion of the galactic
latitude for several latitudes bins.
The standard model described above is unable to describe the profile on
the galactic plane. Still using a $sech^2$ law, but varying the parameters,
a best fit is found for $\beta_\star=122$ pc, a value smaller than the
currently accepted ones. Using an exponential law gives $\beta_\star=204\pm
57$ pc and $\alpha_\star=2.7\pm0.5$ kpc. To obtain a value for $\beta_\star$
closed to the observed in the Solar Neighbourhood, they allow for a
varying $\beta_\star$. Up to 5.3 kpc they keep $\beta_\star=165$ then
they assume a gradient of 30 pc / kpc so that at $R_\odot$
$\beta_\star=247\pm 69$. The corresponding radial scalelengths is
$\alpha_\star=3\pm0.5$ kpc.

In this paper there is also a review of previous determination of 
$\alpha_\star$.
Determination from NIR star counts and diffuse integrated emission gives
shosrt values for the scalelength ($\alpha_\star< 3$ kpc). Optical-based 
measures give $3.5  <\alpha_\star< 5.5 $ kpc. The lower limit is obtained by 
\citet{DeVaucouleursAJ1978} using results on our Galaxy and mean
properties of disks in external galaxies: an extimate of the local vertically 
integrated surface brightness in the B-band is derived from star counts
and compared with a mean central surface brightness 21.65 mag
arcsec$^{-1}$ (Freeman Law). The upper value is derived from the
integrated  blue and red starlight observed by the Background Experiment
on board of {\em Pioneer 10} \citep{VanDerKruitA&A1986}, using a
modified \citet{BahcallApJS1980} model. To avoid region with high
extinction, data for galatic longitude $b > 20^\circ$ only are used: thus,
as shown by the author, only the value $\alpha_\star/\beta_\star$
can be derived. He assumes $\beta_\star=325$ pc. As suggested by 
\citet{KentApJ1991} this method is sensitive to local surface brightness 
gradients and may only give a measure of the local exponential scalelength.
Other determination from the distribution of $IRAS$ OH/IR stars gives 
values from 4.2 to 6. The first measure is anyway obtained excluding the
Galactic equator.

\citet{RobinA&A1992} find the scalelength analyzing B and V-band number
counts of stars up to $m_V=25$ mag in a low absorption window in the direction 
of the Galactic anticenter.  They adopt a disk model that behaves exponentially
in the radial direction and is close to a $sech^2$ in the vertical.
The luminosity function of HR diagram stars is evaluated from a model.
A correction for extinction is evaluated from the U-B/B-V plot of a
smaller sample of stars in their field for which they also have U-band
data. They obtain $\alpha_\star=2.5$ kpc. Number counts for stars with 
$m_V>16$ mag cannot be explained without a truncation in the disk: they
obtain $R_{max}=5.5 \alpha_\star$ \citep[see also][]{RobinApJL1992}.

\section{Galactic vertical scalelength $\beta_\star$}

\citet{BahcallApJS1980} model involves an exponential disk and a de
Vaucouleurs spheroid. Model results are compared with B and V star 
counts at $b>20^\circ$. The disk luminosity function assumed is the one 
for the solar neighborhood, the disk consistent of a mixture of PopI and
PopII stars. The radial scalelength is $\alpha_\star=3.5$
\citep{DeVaucouleursAJ1978}.
Disk scaleheights are derived from several references and
summarized in this way: young stars ($M_V<2$) have $\beta_\star=90$ pc,
old disk dwarfs ($M_V>5$) have $\beta_\star=325$ pc, while a linear relation
for stars in the range $2<M_V<5$ is assumed. In this formalism giants 
have $\beta_\star=250$ pc. 
In a subsequent work \citep{BahcallApJS1984}, limits are put on the
scalelengths, after exploring several values and comparing the model to
new starcounts: $\beta_\star=250\pm100$ pc for giants and 
$\beta_\star=350\pm50$ pc for old disk dwarfs. Althought data are
poorly sensible to $\alpha_\star$, data can be reasonably fit only for 
$\alpha_\star>2.5$ kpc.

\citet{WainscoatApJS1992} makes a model of the galaxy to fit starcounts
from 12-$\mu m$ and 25-$\mu m$ data in the {\em IRAS} Point Source Catalog.
The disk is simulated with a standard double exponential, and features
like spirals, bar and ring are added. There are also a bulge and a
stellar halo.
The radial scalelength is the same $\alpha_\star=3.5$ kpc, with the
bulge truncated at 15 kpc.
The luminosity function is calculated from a compilation of 87 types of
galactic sources responsible for emission in the NIR bands. Scaleheights
for each of the sources, classified by their spectral type, are similar 
to the \citet{BahcallApJS1980} one (e.g. the old disk component has 
$\beta_\star=325$ pc etc.).
A previous model to fit K-band star count and 12-$\mu m$  IRAS source
count (\citealt{GarwoodPASP1987}, see also \citealt{JonesMNRAS1981})
was using slightly smaller values ($\beta_\star=300$ pc for old disk
dwarfs).

Recently \citet*{HaywoodA&A1997a,HaywoodA&A1997b} have questioned the
validity of the exponential assumption for the vertical structure.
In their model (much more complicate!), the vertical structure of the 
disk results from the combined effect of the Star Formation history and 
of the secular heating of the disk (copiato!), rather than assuming 
different values of $\beta_\star$ for different component. After testing 
their model with observed starcounts in B, V and I, they claim that a single 
exponential is unsuitable to describe well data for $z<500$ pc. They say 
that the vertical density distribution decreases faster than the
$300-350$ pc generally assumed. In \citet{RuphyA&A1996} a value of
$250$ pc is suggested. They use $\alpha_\star=2.5$ kpc
\citep{RuphyA&A1996}.  The model includes also a thick disk.


==> program/spiral.tex <==
\section{scalelengths in spiral galaxies}
\citet{PeletierA&AS1994} have compared B and K-band disk scalelengths for 
a diameter limited sample of 37 Sb-Sc galaxies with a uniform distribution of 
orientation respect to the sky. Their aim is to separate in 
$\alpha_B/\alpha_K$ the effects of extinction from those of a change in 
stellar population (only the former being dependent on the inclination of 
the galaxy). From the metallicity gradients a ratio of 1.17 is extimated, 
independent of inclination, while the observed values goes from 1.3 for 
face-on galaxies to 1.7 for edge-on \citep{PeletierA&A1995}. 
Moreover they observe from a previous work that in dust-free late type 
galaxies the ratio between scalelengths is small: 
$\alpha_B/\alpha_I=1.04\pm0.05$, equivalent to $\alpha_B/\alpha_K=1.08\pm0.1$ 
for almost any stellar population model. Thus they claim that the
change in scalelength with $\lambda$ is due to dust extinction.
Their data can only be fitted with a radiative transfer model where the 
dust scalelength is bigger than twice the stellar, althought a suggestion 
is made that this result can change if scattering and clumping are
included in the analysis. A central face-on B-band optical depth of 2-3 
is extimated. {\bf They also try with a two component model for the
dust}

For a sample of 86 face-on galaxies \citet{DeJongA&A1996b} finds 
$\alpha_B/\alpha_K=1.22\pm0.23$, a value compatible with 
\citet{PeletierA&AS1994} analysis. Comparing color-color plots with
Monte Carlo radiative transfer models he concludes that dust can't be 
responsible for the gradient in color, that he suggests being caused
by a change in stellar population in the outer parts of the disk.

\citet{DeGrijsA&AS1996} have analized the structure of eight large
edge-on galaxies in the UGC catalog using BVRI CCD images.
Fitting an exponential function to the vertical profile, they
find a scaleheight 130 and 330 pc (values corrected to
$H_0$=75 km s$^{-1}$ Mpc$^{-1}$).
In some late type spiral an additional thick disk is needed.
No clear trend of scaleheights variation with passband is observed.
As for the radial scalelength, they observe a ratio $\alpha_B/\alpha_I= 
1.17\pm0.1$, consistent with~\citet{PeletierA&AS1994} values. 
No trend with galactic type is observed.
The ratio between the radial and the vertical scalelength in the I-band
for region less affected by dust, is 
$\alpha_\star/\beta_\star=11.8\pm0.8$, consistent with $9.4\pm3.6$ 
from \citet{VanDerKruitA&A1982}.
%but small compared to the theoretical value of about 10 necessary 
%to fit the maximum rotational velocity of disk-dominated Sc 
%galaxies~\citep{BottemaA&A1983}. 
%The value for our galaxy from \citet{VanDerKruitA&A1986} is 8.5.
{\bf to remember: an exponential bulge is used for some galaxies.
Their mean value is 2.66 for the I band with Ho=75.
their scalelength is the projected one, not the intrinsic: in a 
transparent edge-on case the projected scalelength is 10\% of
the intrinsic one, so the ratio $\alpha_\star/\beta_\star$ should
be reduced by 10\%, not augmented like they say.}

\citet*{MoriondoA&AS1998} finds a mean scalelength $\alpha_\star\approx=3 $ kpc
(when corrected to H$_0$=75 km s$^{-1}$ Mpc$^{-1}$)  in both J and K-band.

